SPFresh: Incremental In-Place Update for Billion-Scale Vector Search

Approximate Nearest Neighbor Search (ANNS) is now widely used in various applications, ranging from information retrieval, question answering, and recommendation, to search for similar high-dimensional vectors. As the amount of vector data grows continuously, it becomes important to support updates to vector index, the enabling technique that allows for efficient and accurate ANNS on vectors. Because of the curse of high dimensionality, it is often costly to identify the right neighbors of a single new vector, a necessary process for index update. To amortize update costs, existing systems maintain a secondary index to accumulate updates, which are merged by the main index by global rebuilding the entire index periodically. However, this approach has high fluctuations of search latency and accuracy, not even to mention that it requires substantial resources and is extremely time-consuming for rebuilds. We introduce SPFresh, a system that supports in-place vector updates. At the heart of SPFresh is LIRE, a lightweight incremental rebalancing protocol to split vector partitions and reassign vectors in the nearby partitions to adapt to data distribution shift. LIRE achieves low-overhead vector updates by only reassigning vectors at the boundary between partitions, where in a high-quality vector index the amount of such vectors are deemed small. With LIRE, SPFresh provides superior query latency and accuracy to solutions based on global rebuild, with only 1% of DRAM and less than 10% cores needed at the peak compared to the state-of-the-art, in a billion scale vector index with 1% of daily vector update rate.

==> related-works.tex <==
\section{Related works}
\yuming{highly overlapped with background}
\label{sect:related}
\subsection{Approximate Nearest Neighbor Search (ANNS).}
Many ANNS approaches in the literature focusing on the high recall and low latency solutions. They build ANNS indices to effectively organize data and serve search queries. They can be divided into two categories: in-memory ANNS indices and disk-based ANNS indices.

In-memory ANNS indices include hash-based methods~\cite{Datar:2004:LHS,He:2010:SSS,Jain:2008:Learned,kulis2009kernelized,raginsky2009locality,wang2010semi,mu2010non,song2011multiple,weiss2009spectral,xu2011complementary} which use multiple locality-preserved hash functions to do the vector to partition mapping, space partition tree based methods~\cite{BentleyCACM1975,FreidmanTOMS1977,BeisCVPR1997,SproullALGO1991,YianilosSODA1993,AryaJACM1998,MooreUAI2000,LiuNIPS2004,NisterCVPR2006,DasguptaSTOC2008,McCartin-LimICML12,WangPAMI2014,MujaPAMI2014,BabenkoCVPR17} which use tree to represent the space division and the vector to subspaces mapping, neighborhood graph based methods~\cite{HajebiASZ11,DongCL11,WangWZTGL12,zbMATH03016052,toussaint1980relative,gabriel1969new,FuNSG17,malkov2016efficient} which organize all the vectors into a neighborhood graph with each vector connected to its nearest vectors, quantization-based methods~\cite{jegou2011searching,baranchuk2018revisiting,zhang2019grip,babenko2014inverted,FAISS2020} which use Product Quantization(PQ)~\cite{jegou2010product} to compress the vectors and KMeans to generate the vector to partition mapping codebooks, and hybrid methods~\cite{wang2012query, SPTAG2018, NGTONNG2018, NGTPANNG2016} which consist of space partition trees and a neighborhood graph to take advantage of both tree and graph data structures. These indices store both data and index in memory which cannot satisfy the requirement of large scale datasets.

%\textbf{Hash based methods.} Locality sensitive hashing (LSH)~\cite{Datar:2004:LHS} is the most widely used hash based solution. It uses multiple hash functions to do the vector mapping. For each hash function, vectors that are close in the space are more likely to be hashed to the same bucket than those far away vectors. When a query comes, it first hashes the query to buckets that contain it and then retrieves the elements stored in these buckets. There are many work focusing on finding good hashing functions.~\cite{}

%\textbf{.} The space partition tree based methods try to divide the vector space into subspaces and then use tree to represent the division and subspaces. There are many kinds of space partition trees.\cite{}

%\textbf{.} The nearest neighborhood graph based methods try to organize all the vectors into a graph with each vector connected to its nearest ones, such as KNN graph (KNG)~~\cite{HajebiASZ11,DongCL11,WangWZTGL12}, Delaunay graph (DG) ~\cite{zbMATH03016052}, Relative neighborhood graph (RNG) ~\cite{toussaint1980relative}, Gabriel graph (GG) ~\cite{gabriel1969new}, etc. NSG~\cite{FuNSG17} is a kind of RNG.  HNSW~\cite{malkov2016efficient} is also organized as hierarchical RNGs.

%\textbf{Hybrid methods.} There are also some hybrid methods, such as query-driven iterative search~\cite{wang2012query}, etc. It uses multiple kd-trees to do the navigation and a KNN graph to do the search. SPTAG~\cite{SPTAG2018} improves it by replacing the multiple kd-trees with a balanced KMeans tree as the routing index to do the coarse-grained seed search and use a relative neighborhood graph as the fine-grained search index which has better connectivity.

As the data scale increases, some disk-based ANNS indices have been proposed to efficiently support vector search on billion-scale datasets. They can be divided into graph-based indices and partition-based indices. DiskANN\cite{DISKANN2019NEURIPS} and HM-ANN\cite{HMANN2020NEURIPS} are graph-based solutions. 
DiskANN stores PQ compressed vectors in memory and the navigating spread-out graph along with the full-length vectors on the disk. HM-ANN adapts the popular HNSW algorithm with hierarchical heterogeneous memory, which puts the elements with the highest degrees in the DRAM and maintaining navigable small world graph in the persistent memory. SPANN~\cite{ChenW21} is an partition-based memory-disk hybrid solution which keeps the centroids of the posting lists in memory and large posting lists data on disk. SPANN uses hierarchical balanced clustering and RNG rule~\cite{toussaint1980relative} to optimize cluster assignment.

The above algorithms can support fast high-recall search and thus are widely used. However, almost none of them can support fresh update well as introduced in \S\ref{sect:bg:challenges}.

\subsection{Fresh update support.}
Vearch\cite{VEARCH2018MIDDLEWARE} supports in-place update base on inverted index. Full index must be rebuilt periodically since with the modification of the data, the distribution of the data has changed, and the accuracy and performance of query results will decrease. It is necessary to rebuild the index based on the current distribution using the k-means algorithm. ADBV\cite{ADBV2020VLDB} and Milvus\cite{MILVUS2021SIGMOD} support update by adopting the idea of LSM-tree. ADBV uses VGPQ to store the baseline data, HNSW to store the incremental data and a bitset to track data has been deleted. ADBV periodically merge them to recreate the baseline index. Milvus inserts the most recent data into the memory as MemTable. When MemTable reaches a certain size, it will be written to disk as a new segment. Segments will be continuously merged to optimize queries and delete data. Read amplification:  for search queries, both ADBV and Milvus need to retrieve multiple indices or segments and merge the results, resulting in higher query latency. Write amplification: data needs to be merged and rebuilt many times, which brings a lot of storage space and computing resources overhead.



% \section{Related worksV2}
% For fresh-ANNS, there are a lots of metrics need to be considered.
% \begin{itemize}
%     \item Billion-level Vector Scale : for a single machine with 32GB/64GB, whether it can hold billion-level dataset whose size is hundreds of GBs.
%     \item Query Throughput : although some of the ANN system can reach millseconds-latency, they need to dispatch multiple threads to parallize single query, which makes it decrease the throughput of the system with given cores.
%     \item Search Latency : for ANN systems/indices, one of the most things we care about is latency, whether this system can reach millseconds-latency search(10ms~)
%     \item High Accuracy : whether this system/indice can provide high accuracy(90\%~) in a latency budget (10ms~)
%     \item Index Quality After Update : whether it will get similar performance and accuracy compared to global rebuild indices after update, no count for the indices/systems which can't get high accuracy from statically-built ones.
%     \item Avoid Global Rebuild : some systems can still maintain accuracy, however, some systems only allow fixed update size due to design or memory footprint reasons. Involved global rebuild will result in black window or cost extra double even more times memory/computation resource to keep service online.
% \end{itemize}

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
%     \hline
%      & & \multicolumn{3}{c|}{Indice} & \multicolumn{5}{c|}{System} \\
%      \hline
%      & & SRS & Graph-based & HD-Index & Vearch & PLSH & ADBV & Milvus & SPFresh\\
%      \hline
%       \multirow{2}{*}{Performance} & 
%      Search Latency & $\downarrow$ & $\bullet$ & $\downarrow$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$\\
%       & Query Throughput & $\downarrow$ & $\bullet$ & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\bullet$\\
%      \hline
%      \multirow{2}{*}{Accuracy}
%      & Accuracy In Latency Limit & $\bullet$ & $\downarrow$ & $\bullet$ & $\downarrow$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$\\
%      & Avoid Global Rebuild & $\bullet$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\bullet$\\
%      \hline
%      Scale& 
%      Vector Capacity & $\bullet$ & $\downarrow$ & $\bullet$ & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\bullet$\\
%      \hline
%     \end{tabular}
%     \caption{Latency-Accuracy-Scale Tradeoff in Fresh-ANNS}
%     \label{related_work_table}
% \end{table*}
